Two generalizations of shininess

Shininess is one of the main theory combination methods in Satisfiability Modulo Theories. We present two infinite families of generalizations of it: one involving a property between gentleness and shininess, which helps us see gentleness itself as a variation of shininess; and another having no further computability requirements on the weaker theory, in addition dropping the need for smoothness. We prove these methods sharp, and compare them with existing methods.

==> mycommands.tex <==
\newcommand{\s}{\ensuremath{\sigma}}

\newcommand{\shA}{\ensuremath{\hat{\sA}}}

\newcommand{\shAp}{\ensuremath{(\hat{\sA})^{\prime}}}

\renewcommand{\S}{\ensuremath{\mathcal{S}}}

\renewcommand{\P}{\ensuremath{\mathcal{P}}}

\newcommand{\ax}{\textit{Ax}}

\newcommand{\wit}{\textit{wit}}

\newcommand{\overarrow}{\overrightarrow}

\newcommand{\e}{\sigma_{e}}

\renewcommand{\v}{\sigma_{v}}

\newcommand{\Fo}{\mathbb{F}}

\newcommand{\Tr}{\mathbb{T}}

\newcommand{\wrt}{\textit{w.r.t.} }

\newcommand{\kn}{\kappa}

\newcommand{\free}{\textit{freevars}}

\newcommand{\Ap}{\ensuremath{\A^{\prime}}}

\newcommand{\Bp}{\ensuremath{\B^{\prime}}}

\newcommand{\sAp}{\ensuremath{\sA^{\prime}}}

\newcommand{\sBp}{\ensuremath{\sB^{\prime}}}

\newcommand{\Exists}[1]{\exists\,#1.\:}

\newcommand{\Forall}[1]{\forall\,#1.\:}

\newcommand{\Q}[2]{Q_{#1}\,#2.}

\newcommand{\saa}[1]{S^{\A}_{#1\aleph_{0}}}

\newcommand{\sasa}[1]{S^{\sA}_{#1\aleph_{0}}}

\newcommand{\Saa}[1]{\S^{\A}_{#1\aleph_{0}}}

\newcommand{\Sasa}[1]{\S^{\sA}_{#1\aleph_{0}}}

\newcommand{\sa}[2]{S^{#1}_{#2\aleph_{0}}}

\renewcommand{\t}{\tau}

\newcommand{\Sigmadag}{\Sigma^{\dag}}

\newcommand{\sAdag}{\sA^{\dag}}

\newcommand{\sBdag}{\sB^{\dag}}

%\newcommand{\For}[1]{For(#1)}

\newcommand{\CB}[1]{{\color{red}CB: #1}}

\newcommand{\BP}[1]{{\color{red}BP: #1}}

\newcommand{\GT}[1]{{\color{red}GT: #1}}

\newcommand{\A}{\ensuremath{\mathcal{A}}}

\newcommand{\B}{\ensuremath{\mathcal{B}}}

\newcommand{\C}{\ensuremath{\mathcal{C}}}

\newcommand{\D}{\ensuremath{\mathcal{D}}}

\newcommand{\sA}{\ensuremath{\mathbb{A}}}

\newcommand{\sB}{\ensuremath{\mathbb{B}}}

\newcommand{\sC}{\ensuremath{\mathbb{C}}}

\newcommand{\sD}{\ensuremath{\mathbb{D}}}

\newcommand{\sE}{\ensuremath{\mathbb{E}}}

\newcommand{\sF}{\ensuremath{\mathbb{F}}}

\newcommand{\M}{\ensuremath{\mathcal{M}}}

\newcommand{\F}{\ensuremath{\mathcal{F}}}

\newcommand{\T}{\ensuremath{\mathcal{T}}}

\renewcommand{\S}{\ensuremath{\mathcal{S}}}

\renewcommand{\P}{\ensuremath{\mathcal{P}}}

\newcommand{\G}{\ensuremath{gentle}}

\newcommand{\vars}{\textit{vars}}

\renewcommand{\v}{\sigma_{v}}

\newcommand{\yz}[1]{{\color{blue}yz:{#1}}}

\newcommand{\gt}[1]{{\color{blue}gt:{#1}}}

\newcommand{\bp}[1]{{\color{blue}BP: {#1}}}

\newcommand{\dash}{\vdash}

\newcommand{\tdash}{\vdash_{\T}}

\renewcommand{\t}{\tau}

\newcommand{\nset}[2]{\ensuremath{P_{#2}(#1)}}

\newcommand{\minmods}[2]{\ensuremath{\mathrm{minmods}_{#1, #2}}}

\newcommand{\N}{\ensuremath{\mathbb{N}_{\omega}}}

\newcommand{\qf}[1]{\ensuremath{QF(#1)}}

\newcommand{\eq}[1]{\ensuremath{Eq(#1)}}

\newcommand{\adds}[1]{\ensuremath{(#1)^{2}}}

\newcommand{\addf}[1]{\ensuremath{(#1)_{s}}}

\newcommand{\subf}[1]{\ensuremath{\texttt{0}(#1)}}


\newcommand{\subff}[1]{\ensuremath{#1_{\texttt{0}}}}

\newcommand{\addfs}[1]{\ensuremath{s(#1)}}

\newcommand{\subs}[1]{\ensuremath{#1_{1}}}

\newcommand{\minmod}{\ensuremath{\mathrm{minmod}}}

\newcommand{\minimal}{\ensuremath{\textbf{minimal}}}

\newcommand{\Teven}{\ensuremath{\T_{even}^{\infty}}}

\newcommand{\Tninfty}{\ensuremath{\T_{n,\infty}}}
\newcommand{\cvciii}{\ensuremath{\textsf{CVC3}}}
\newcommand{\cvcfour}{\ensuremath{\textsf{CVC4}}}
\newcommand{\cvcfive}{\ensuremath{\textsf{cvc5}}}

\newcommand{\bb}{\ensuremath{\varsigma}}

\newcommand{\Tbb}{\ensuremath{\T_{\bb}}}

\newcommand{\SI}{\ensuremath{\textbf{SI}}}

\newcommand{\SF}{\ensuremath{\textbf{SF}}}

\newcommand{\SM}{\ensuremath{\textbf{SM}}}

\newcommand{\CV}{\ensuremath{\textbf{CV}}}

\newcommand{\FW}{\ensuremath{\textbf{FW}}}

\newcommand{\SW}{\ensuremath{\textbf{SW}}}

\newcommand{\CM}{\ensuremath{\textbf{CM}}}

\newcommand{\Tone}{\ensuremath{\T_{\mathrm{I}}}}

\newcommand{\Tgeqn}{\ensuremath{\T_{\geq n}}}

\newcommand{\Tinfty}{\ensuremath{\T_{\infty}}}

\newcommand{\Tleqone}{\ensuremath{\T_{\leq 1}}}

\newcommand{\Tleqn}{\ensuremath{\T_{\leq n}}}

\newcommand{\Tmn}{\ensuremath{\T_{\langle m,n\rangle}}}

\newcommand{\Tbbs}{\ensuremath{\T^{s}_{\bb}}}

\newcommand{\Tbbeq}{\ensuremath{\T^{=}_{\bb}}}

\newcommand{\Tbbtwo}{\ensuremath{\T^{2}_{\bb}}}

\newcommand{\Tbbvee}{\ensuremath{\T^{\vee}_{\bb}}}

\newcommand{\Tbbveeeq}{\ensuremath{\T^{=}_{\bb\vee}}}

\newcommand{\Tbbinfty}{\ensuremath{\T^{\infty}_{\bb}}}

\newcommand{\Tonebb}{\ensuremath{\T^{\bb}_{1}}}

\newcommand{\Tbboneneq}{\ensuremath{\T^{\neq}_{\bb,1}}}

\newcommand{\Tbbinftythree}{\ensuremath{\T^{\infty,3}_{\bb}}}

\newcommand{\Tbbneqinfty}{\ensuremath{\T^{\infty}_{\bb\neq}}}

\newcommand{\Tmnbb}{\ensuremath{\T^{\bb}_{m,n}}}

\newcommand{\Tnbb}{\ensuremath{\T^{\bb}_{n}}}

\newcommand{\Tbbneq}{\ensuremath{\T^{\bb}_{n}}}

\newcommand{\Ttwothree}{\ensuremath{\T_{2,3}}}

\newcommand{\addnc}[1]{\ensuremath{(#1)_{\vee}}}

\newcommand{\Tupinfty}{\ensuremath{\T^{\infty}}}

\newcommand{\TM}{\ensuremath{\T_{f}}}

\newcommand{\TsM}{\ensuremath{\T^{s}_{f}}}

\newcommand{\Tmninfty}{\ensuremath{\T^{\infty}_{m,n}}}

\newcommand{\Toneinfty}{\ensuremath{\T^{\infty}_{1}}}

\newcommand{\Ttwoinfty}{\ensuremath{\T^{\infty}_{2}}}

\newcommand{\Toneinftyneq}{\ensuremath{\T_{1,\infty}^{\neq}}}

\newcommand{\Ttwoinftyneq}{\ensuremath{\T_{2,\infty}^{\neq}}}

\newcommand{\Toneodd}{\ensuremath{\T_{1}^{odd}}}

\newcommand{\Toddneq}{\ensuremath{\T_{odd}^{\neq}}}

\newcommand{\Ttwothreethree}{\ensuremath{\T_{2,3}^{3}}}

\newcommand{\Tnequpinfty}{\ensuremath{\T^{\infty}_{\neq}}}

\newcommand{\Ttwo}{\ensuremath{\T_{\mathrm{II}}}}

\newcommand{\Tthree}{\ensuremath{\T_{\mathrm{III}}}}

\newcommand{\Tfour}{\ensuremath{\T_{\mathrm{IV}}}}

\newcommand{\Tfive}{\ensuremath{\T_{\mathrm{V}}}}

\newcommand{\addsi}[2]{\ensuremath{#1_{\texttt{+}#2}}}

\newcommand{\Tsix}{\ensuremath{\T_{\mathrm{VI}}}}

\newcommand{\Tthreeone}{\ensuremath{\T^{3}_{\mathrm{I}}}}

\newcommand{\Tseven}{\ensuremath{\T_{\mathrm{VII}}}}

\newcommand{\Teight}{\ensuremath{\T_{\mathrm{VIII}}}}

\newcommand{\Tnine}{\ensuremath{\T_{\mathrm{IX}}}}

\newcommand{\Tten}{\ensuremath{\T_{\mathrm{X}}}}

\newcommand{\Televen}{\ensuremath{\T_{\mathrm{XI}}}}

\newcommand{\Tthreetwo}{\ensuremath{\T^{3}_{\mathrm{II}}}}

\newcommand{\Ttwelve}{\ensuremath{\T_{\mathrm{XII}}}}

\newcommand{\Tthirteen}{\ensuremath{\T_{\mathrm{XIII}}}}

\newcommand{\Tfourteen}{\ensuremath{\T_{\mathrm{XIV}}}}

\newcommand{\Tfifteen}{\ensuremath{\T_{\mathrm{XV}}}}

\newcommand{\Tsixteen}{\ensuremath{\T_{\mathrm{XVI}}}}

\newcommand{\Tseventeen}{\ensuremath{\T_{\mathrm{XVII}}}}

\newcommand{\Teighteen}{\ensuremath{\T_{\mathrm{XVIII}}}}

\newcommand{\smooth}{\textbf{SM}}

\newcommand{\stainf}{\textbf{SI}}

\newcommand{\convex}{\textbf{CV}}

\newcommand{\finwit}{\textbf{FW}}

\newcommand{\strfinwit}{\textbf{SW}}

\newcommand{\stafin}{\textbf{SF}}

\newcommand{\finmodpro}{\textbf{FM}}

\newcommand{\cmmf}{\textbf{CF}}

\renewcommand{\S}{\ensuremath{\mathcal{S}}}

\renewcommand{\P}{\ensuremath{\mathcal{P}}}

\newcommand{\NEQ}{\ensuremath{\neq}}

%\newcommand{\replete}{replete }

\newcommand{\NNEQ}[1]{\ensuremath{\neq(#1_{1},\ldots,#1_{n})}}

\newcommand{\NNNEQ}[2]{\ensuremath{\neq(#1_{1},\ldots,#1_{#2})}}

\newcommand{\inj}{\ensuremath\mathit{inj}\xspace}

\newcommand{\sur}{\ensuremath\mathit{sur}\xspace}

%\newcommand{\email}[1]{\href{mailto:#1}{#1}}

\newcommand{\dif}[1]{\ensuremath{\psi^{orb}_{\geq #1}}}

\newcommand{\orb}[1]{\ensuremath{\psi^{orb}_{=#1}}}

\newcommand{\eqs}{{\scaleobj{0.7}{=}}}

\newcommand{\difs}{\scaleobj{0.7}{\neq}}

\newcommand{\distinct}[1]{\NNEQ{x}}

\renewcommand{\int}[2]{\mathcal{#1}/\mathcal{#2}}

\newcommand{\Tp}{\ensuremath{\T_{P}^{\nf}}}

\newcommand{\Tot}{\ensuremath{\T_{\textit{orb}}^{2}}}

\newcommand{\To}{\ensuremath{\T_{\textit{orb}}}}

\newcommand{\Tle}{\ensuremath{\T_{\leq}}}

\newcommand{\Tgr}{\ensuremath{\T_{\geq}}}

\newcommand{\Tgp}{\ensuremath{\T_{\leq}^{orb}}}

\newcommand{\Sp}{\ensuremath{\Sigma_{P}}}

\newcommand{\Spn}{\ensuremath{\Sigma_{P}^{\mathbb{N}}}}

\newcommand{\Spnn}{\ensuremath{\Sigma_{P}^{\mathbb{N} \times \mathbb{N}}}}

\newcommand{\Tpt}{\ensuremath{\T_{P}^{\nft}}}

\newcommand{\phieqs}{\ensuremath{\varphi^{\eqs}_{\geq n}}}

\newcommand{\Tb}{\ensuremath{\T_{\infty}^{\nf}}}

%\newcommand{\reference}{~(see  \Cref{theo:testtheories})}
\newcommand{\reference}{}

\newcommand{\No}{\ensuremath{\mathbb{N}^{*}}}

\newcommand{\Sone}{\ensuremath{\Sigma_{1}}}

\newcommand{\Inf}{\ensuremath{\aleph_{0}}}

\newcommand{\nop}[1]{\ensuremath{\textit{sub}(#1)}}

\newcommand{\eqp}[1]{\ensuremath{Eq^{\prime}(#1)}}

\newcommand{\eqpp}[1]{\ensuremath{Eq^{\prime\prime}(#1)}}

\newcommand{\spec}{\ensuremath{\textit{Spec}}}

\newcommand{\dom}[1]{\ensuremath{dom(#1)}}

\newcommand{\ns}{\ensuremath{t}}

\newcommand{\os}{\ensuremath{s}}

\newcommand{\nf}{\ensuremath{h}}

\newcommand{\nft}{\ensuremath{g}}

\newcommand{\of}{\ensuremath{f}}

\newcommand{\OF}{\ensuremath{F}}

\newcommand{\NF}{\ensuremath{H}}

\newcommand{\Ss}{\ensuremath{\Sigma_{s}}}

\newcommand{\Sat}{\ensuremath{\Sigma_{t}^{a}}}

\newcommand{\TMn}{\ensuremath{\T_{\nft}}}

\newcommand{\NFT}{\ensuremath{G}}

\newcommand{\quagen}{$\mathfrak{F}$-QG}

\newcommand{\coquagen}{co-$\mathfrak{F}$-QG}

\newcommand{\csi}{computable and stably infinite}

\newcommand{\quacom}{right-computable}

\newcommand{\rc}{right-computable}

\newcommand{\TPbb}{\ensuremath{\T^{P}_{\alpha}}}

\newcommand{\TPnbb}{\ensuremath{\T^{P_{n}}_{\beta}}}

\newcommand{\Quagen}{$\mathfrak{F}$-QG}

\newcommand{\Coquagen}{Co-$\mathfrak{F}$-QG}

\newcommand{\Csi}{Computable and stably infinite}

\newcommand{\Quacom}{Right-computable}

\newcommand{\Rc}{Right-computable}

\newcommand{\Cqg}{Computable and \quagen{}}

\newcommand{\cqg}{computable and \quagen{}}

\newcommand{\Com}{Computable}

\newcommand{\com}{computable}

\newcommand{\weagen}{left-computable}

\newcommand{\Weagen}{Left-computable}

\newcommand{\lc}{left-computable}

\newcommand{\Lc}{Left-computable}

\newcommand{\TPeven}{\ensuremath{\T^{P}_{even}}}

\newcommand{\Tgrinf}{\ensuremath{\T^{\infty}_{\leq}}}

\newcommand{\QUAGEN}{\textbf{QG}}

\newcommand{\CSI}{\textbf{C+SI}}

\newcommand{\QUACOM}{\textbf{RC}}

\newcommand{\RC}{\textbf{RC}}

\newcommand{\CQG}{\textbf{C+QG}}

\newcommand{\COM}{\textbf{CS}}

\newcommand{\WEAGEN}{\textbf{LC}}

\newcommand{\LC}{\textbf{LC}}

\newcommand{\GEN}{\textbf{GE}}

\newcommand{\SHI}{\textbf{S}}

\newcommand{\CFS}{\textbf{CFS}}

\newcommand{\DEC}{\textbf{D}}

\newcommand{\CSM}{\textbf{CSM}}

\newcommand{\ID}{\textbf{ID}}

\newcommand{\Tgralpha}{\ensuremath{\T^{\alpha}_{\leq}}}

\newcommand{\enu}{enumerable}

\newcommand{\Enu}{Enumerable}

\newcommand{\ENU}{\textbf{E}}

\newcommand{\cofin}{co-finite}

\newcommand{\Cofin}{Co-finite}

\newcommand{\COFIN}{\textbf{C-F}}

\newcommand{\maxmod}[1]{\ensuremath{\textbf{maxmod}(#1)}}

\newcommand{\List}[1]{\ensuremath{\textit{list}(#1)}}

\newcommand{\Tmin}{\ensuremath{\T_{-}}}

\newcommand{\Th}[1]{\ensuremath{\T_{\langle\scriptscriptstyle #1\rangle}}}

\newcommand{\Comspe}{Computable spectra}

\newcommand{\comspe}{computable spectra}

\newcommand{\EL}{\ensuremath{\mathcal{EL}}}


\newcommand{\Test}[1]{\ensuremath{\T_{\texttt{#1}}}}

\newcommand{\algofont}[1]{\textnormal{\textsc \selectfont\sffamily  #1}}
\newcommand{\procform}{\algofont{ProcessFormula}}
\newcommand{\procnum}{\algofont{ProcessNumber}}

\newcommand{\Teq}{\ensuremath{\T_{\scriptscriptstyle\textbf{eq}}}}

\newcommand{\class}[1]{\ensuremath{\mathfrak{T}_{\text{#1}}}}

\newcommand{\omg}[1]{\ensuremath{#1_{\omega}}}

\newcommand{\Testsi}{\ensuremath{\T_{>n}^{P}}}

\newcommand{\Testcfs}{\ensuremath{\T_{=}^{P}}}

\newcommand{\Testsm}{\ensuremath{\T^{n}_{m}}}

\newcommand{\Testg}{\ensuremath{\T_{\leq}^{S}}}

\newcommand{\Testmm}{\ensuremath{\T_{\geq}^{P}}}

\newcommand{\Teqn}{\ensuremath{\T_{=n}}}

\newcommand{\Sigmasigma}{\ensuremath{Sig^{P}_{\Sigma}}}

\newcommand{\Gal}{\ensuremath{G}}

\newcommand{\unc}{\ensuremath{U}}

\endinput
